SinGAN-Seg: Synthetic training data generation for medical image segmentation

Analyzing medical data to find abnormalities is a time-consuming and costly task, particularly for rare abnormalities, requiring tremendous efforts from medical experts. Artificial intelligence has become a popular tool for the automatic processing of medical data, acting as a supportive tool for doctors. However, the machine learning models used to build these tools are highly dependent on the data used to train them. Large amounts of data can be difficult to obtain in medicine due to privacy, expensive and time-consuming annotations, and a general lack of data samples for infrequent lesions. Here, we present a novel synthetic data generation pipeline, called SinGAN-Seg, to produce synthetic medical images with corresponding masks using a single training image. Our method is different from the traditional GANs because our model needs only a single image and the corresponding ground truth to train. Our method produces alternative artificial segmentation datasets with ground truth masks when real datasets are not allowed to share. The pipeline is evaluated using qualitative and quantitative comparisons between real and synthetic data to show that the style transfer technique used in our pipeline significantly improves the quality of the generated data and our method is better than other state-of-the-art GANs to prepare synthetic images when the size of training datasets are limited. By training UNet++ using both real and the synthetic data generated from the SinGAN-Seg pipeline, we show that models trained with synthetic data have very close performances to those trained on real data when the datasets have a considerable amount of data. In contrast, Synthetic data generated from the SinGAN-Seg pipeline can improve the performance of segmentation models when training datasets do not have a considerable amount of data. The code is available on GitHub.

==> figure_text/random_samples.tex <==
\begin{figure*}
    \centering
    \newcommand{\imgwidth}{0.15\textwidth}
    \includegraphics[width=\imgwidth, height=\imgwidth]{figures/gen_samples/102_img.jpg}
    \includegraphics[width=\imgwidth, height=\imgwidth]{figures/gen_samples/chk_id_102_gen_scale_0_0_img.png}
    \includegraphics[width=\imgwidth, height=\imgwidth]{figures/gen_samples/chk_id_102_gen_scale_0_1_img.png}
    \includegraphics[width=\imgwidth, height=\imgwidth]{figures/gen_samples/chk_id_102_gen_scale_0_2_img.png}
    \includegraphics[width=\imgwidth, height=\imgwidth]{figures/gen_samples/chk_id_102_gen_scale_0_3_img.png}
    \includegraphics[width=\imgwidth, height=\imgwidth]{figures/gen_samples/chk_id_102_gen_scale_0_4_img.png}
    
    \includegraphics[width=\imgwidth, height=\imgwidth]{figures/gen_samples/102_mask.jpg}
    \includegraphics[width=\imgwidth, height=\imgwidth]{figures/gen_samples/chk_id_102_gen_scale_0_0_mask.png}
    \includegraphics[width=\imgwidth, height=\imgwidth]{figures/gen_samples/chk_id_102_gen_scale_0_1_mask.png}
    \includegraphics[width=\imgwidth, height=\imgwidth]{figures/gen_samples/chk_id_102_gen_scale_0_2_mask.png}
    \includegraphics[width=\imgwidth, height=\imgwidth]{figures/gen_samples/chk_id_102_gen_scale_0_3_mask.png}
    \includegraphics[width=\imgwidth, height=\imgwidth]{figures/gen_samples/chk_id_102_gen_scale_0_4_mask.png}
    
    \includegraphics[width=\imgwidth, height=\imgwidth]{figures/gen_samples/103_img.jpg}
    \includegraphics[width=\imgwidth, height=\imgwidth]{figures/gen_samples/chk_id_103_gen_scale_0_0_img.png}
    \includegraphics[width=\imgwidth, height=\imgwidth]{figures/gen_samples/chk_id_103_gen_scale_0_1_img.png}
    \includegraphics[width=\imgwidth, height=\imgwidth]{figures/gen_samples/chk_id_103_gen_scale_0_2_img.png}
    \includegraphics[width=\imgwidth, height=\imgwidth]{figures/gen_samples/chk_id_103_gen_scale_0_3_img.png}
    \includegraphics[width=\imgwidth, height=\imgwidth]{figures/gen_samples/chk_id_103_gen_scale_0_4_img.png}
    
    \includegraphics[width=\imgwidth, height=\imgwidth]{figures/gen_samples/103_mask.jpg}
    \includegraphics[width=\imgwidth, height=\imgwidth]{figures/gen_samples/chk_id_103_gen_scale_0_0_mask.png}
    \includegraphics[width=\imgwidth, height=\imgwidth]{figures/gen_samples/chk_id_103_gen_scale_0_1_mask.png}
    \includegraphics[width=\imgwidth, height=\imgwidth]{figures/gen_samples/chk_id_103_gen_scale_0_2_mask.png}
    \includegraphics[width=\imgwidth, height=\imgwidth]{figures/gen_samples/chk_id_103_gen_scale_0_3_mask.png}
    \includegraphics[width=\imgwidth, height=\imgwidth]{figures/gen_samples/chk_id_103_gen_scale_0_4_mask.png}
    
    \includegraphics[width=\imgwidth, height=\imgwidth]{figures/gen_samples/118_img.jpg}
    \includegraphics[width=\imgwidth, height=\imgwidth]{figures/gen_samples/chk_id_118_gen_scale_0_0_img.png}
    \includegraphics[width=\imgwidth, height=\imgwidth]{figures/gen_samples/chk_id_118_gen_scale_0_1_img.png}
    \includegraphics[width=\imgwidth, height=\imgwidth]{figures/gen_samples/chk_id_118_gen_scale_0_2_img.png}
    \includegraphics[width=\imgwidth, height=\imgwidth]{figures/gen_samples/chk_id_118_gen_scale_0_3_img.png}
    \includegraphics[width=\imgwidth, height=\imgwidth]{figures/gen_samples/chk_id_118_gen_scale_0_4_img.png}
    
    \includegraphics[width=\imgwidth, height=\imgwidth]{figures/gen_samples/118_mask.jpg}
    \includegraphics[width=\imgwidth, height=\imgwidth]{figures/gen_samples/chk_id_118_gen_scale_0_0_mask.png}
    \includegraphics[width=\imgwidth, height=\imgwidth]{figures/gen_samples/chk_id_118_gen_scale_0_1_mask.png}
    \includegraphics[width=\imgwidth, height=\imgwidth]{figures/gen_samples/chk_id_118_gen_scale_0_2_mask.png}
    \includegraphics[width=\imgwidth, height=\imgwidth]{figures/gen_samples/chk_id_118_gen_scale_0_3_mask.png}
    \includegraphics[width=\imgwidth, height=\imgwidth]{figures/gen_samples/chk_id_118_gen_scale_0_4_mask.png}
    
    \caption{Sample real images and corresponding SinGAN generated synthetic GI-tract images with corresponding masks. The first column is illustrated with real images and masks. All other columns represent randomly generated synthetic data from SinGANs which were trained from the image on the first column. }
    \label{fig:real_vs_fake_polyp_images}
\end{figure*}



==> figure_text/sinGAN_big_picture.tex <==
\begin{figure*}
    \centering
    \includegraphics[width=\textwidth]{figures/SinGAN-polyp-augmentation-big-picture_v2.pdf}
    \caption{The complete pipeline of SinGAN-Seg to generate synthetic segmentation datasets. \textit{Step 1}: represents the training of four channels SinGAN models. \textit{Step 2}: represents fine tuning step using the neural style transfer~\cite{gatys2015neural}. \textit{Four channels SinGAN}: Single training step of our four-channels SinGAN. Note the stacked input and output compared to the original SinGAN implementation ~\cite{shaham2019singan} which input only single image with a noise vector and output only an image. In our SinGAN implementation, all the generators (from $G_0$ to $G_{N-1}$), except $G_N$, get four channels image (a polyp image and a ground truth) as the input in addition to the input noise vector. The first generator, $G_N$ get only the noise vector as the input. The discriminators also get four channels images which consist of a RGB polyp image and a binary mask as input. The inputs to the discriminators can be either real or fake. }
    \label{fig:sinGAN_seg_big_picture}
\end{figure*}

==> figure_text/sinGAN_training.tex <==
\begin{figure}
    \centering
    \includegraphics[width=\columnwidth]{figures/SinGAN-polyp-augmentation-to_paper_training_v3.pdf}
    \caption{singGAN training process. G represents a four-channels SinGAN model.}
    \label{fig:singan_training_process}
\end{figure}

==> glossary.tex <==
\newacronym{gan}{GAN}{generative adversarial network}
\newacronym{ai}{AI}{artificial intelligence}
\newacronym{ml}{ML}{machine learning}
\newacronym{dl}{DL}{deep learning}
\newacronym{ann}{ANN}{artificial neural network}
\newacronym{gi}{GI}{gastrointestinal tract}
\newacronym{svm}{SVM}{support vector machine}
\newacronym{dnn}{DNN}{deep neural network}
\newacronym{cnn}{CNN}{convolutional neural network}
\newacronym{gpu}{GPU}{graphic processing unit}
\newacronym{pypi}{PyPI}{Python package index}
\newacronym{gdpr}{GDPR}{general data protection regulation}
\newacronym{ct}{CT}{computed tomography}
\newacronym{iou}{IOU}{intersection over union}
\newacronym{gbm}{GBM}{glioblastoma multiforme}
\newacronym{mri}{MRI}{Magnetic resonance imaging}

==> tables/fold_average_only_for_polyps.tex <==
\begin{table*}[!t]
\centering

\caption{Three-fold average of basic metrics to compare real vs synthetic performance with UNet++ and the effect of style-transfers performance. $cw:sw$ is the short form of $content:style$ weights ratio. Baseline performance values of using real data are represented using bold text. Moreover, the best performance values of using fake data are marked using bold text.}
\begin{tabular}{llrrrrrr}
\toprule
Train data & ST (cw:sw) & \multicolumn{1}{l}{dice\_loss} & \multicolumn{1}{l}{iou\_score} & \multicolumn{1}{l}{fscore} & \multicolumn{1}{l}{accuracy} & \multicolumn{1}{l}{recall} & \multicolumn{1}{l}{precision} \\
\midrule
\textbf{REAL} & NA & \textbf{0.1123} & \textbf{0.8266} & \textbf{0.8882} & \textbf{0.9671}& \textbf{0.8982} & \textbf{0.9161} \\
\midrule
\multirow{3}{*}{FAKE-1} & No ST & 0.1645 & 0.7617 & 0.8357 & 0.9531 & 0.863 & 0.8793 \\
 & 1:1 & 0.1504 & 0.7782 & 0.85 & 0.9572 & 0.8672 & 0.8917 \\
 & 1:1000 & 0.1473 & 0.782 & 0.853 & 0.9591 & 0.8624 & 0.9005 \\
 \midrule
\multirow{3}{*}{FAKE-2} & No ST & 0.1549 & 0.7729 & 0.8453 & 0.9561 & 0.8692 & 0.8895 \\
 & 1:1 & 0.155 & 0.7765 & 0.8453 & 0.9575 & \textbf{0.8729} & 0.8852 \\
 & 1:1000 & 0.1477 & 0.7854 & 0.8525 & 0.9609 & 0.8647 & 0.9038 \\
\midrule
\multirow{3}{*}{FAKE-3} & No ST & 0.161 & 0.7683 & 0.8391 & 0.9556 & 0.8568 & 0.8945 \\
 & 1:1 & 0.1475 & 0.7845 & 0.8525 & 0.9585 & 0.8723 & 0.8936 \\
 & 1:1000 & 0.1408 & 0.7923 & 0.8593 & 0.9629 & 0.8693 & 0.9078 \\
\midrule
\multirow{3}{*}{FAKE-4} & No ST & 0.1649 & 0.7638 & 0.8352 & 0.9525 & 0.8669 & 0.878 \\
 & 1:1 & 0.1464 & 0.7848 & 0.8537 & 0.9594 & 0.8713 & 0.8921 \\
 & 1:1000 & \textbf{0.137} & \textbf{0.7983} & \textbf{0.863} & \textbf{0.9636} & 0.8653 & 0.9185 \\
\midrule
\multirow{3}{*}{FAKE-5} & No ST & 0.1654 & 0.7668 & 0.8345 & 0.9563 & 0.8565 & 0.8919 \\
 & 1:1 & 0.1453 & 0.7887 & 0.8547 & 0.961 & 0.8703 & 0.9 \\
 & 1:1000 & 0.1458 & 0.7889 & 0.8543 & 0.962 & 0.8527 & \textbf{0.9211} \\
\bottomrule
\end{tabular}
\label{tab:real_vs_synthetic_fold_average}
\end{table*}

==> tables/real_vs_fake_only_iou_for_small_dataset.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[!t]
\centering
\caption{Real vs Fake comparisons for small datasets. The fake images were generated using style tranfer ration $1:1000$.}
\begin{tabular}{llrrrrrr}
\toprule
 &  & \multicolumn{1}{l}{dice\_loss} & \multicolumn{1}{l}{iou\_score} & \multicolumn{1}{l}{fscore} & \multicolumn{1}{l}{accuracy} & \multicolumn{1}{l}{recall} & \multicolumn{1}{l}{precision} \\
\midrule
Real & 5 & 0.4662 & 0.4618 & 0.5944 & 0.8751 & 0.7239 & 0.6305 \\
Fake & 50 & \textbf{0.3063} & \textbf{0.5993} & \textbf{0.7048} & \textbf{0.9211} & \textbf{0.7090} & \textbf{0.8133} \\
\midrule
Real & 10 & 0.3932 & 0.5969 & 0.7079 & 0.9164 & 0.7785 & 0.7516 \\
Fake & 100 & \textbf{0.2565} & \textbf{0.6478} & \textbf{0.7457} & \textbf{0.9259} & \textbf{0.7911} & \textbf{0.7970} \\
\midrule
Real & 15 & 0.2992 & 0.6431 & 0.7402 & 0.9322 & 0.7388 & \textbf{0.8602} \\
Fake & 150 & \textbf{0.2852} & \textbf{0.6559} & \textbf{0.7624} & \textbf{0.9329} & \textbf{0.8172} & 0.7833 \\
\midrule
Real & 20 & 0.3070 & \textbf{0.6680} & \textbf{0.7668} & 0.9328 & \textbf{0.7771} & 0.8566 \\
Fake & 200 & \textbf{0.2532} & 0.6569 & 0.7544 & \textbf{0.9342} & 0.7317 & \textbf{0.8827} \\
\midrule
Real & 25 & \textbf{0.2166} & \textbf{0.6995} & \textbf{0.7929} & 0.9405 & \textbf{0.7955} & 0.8804 \\
Fake & 250 & 0.2182 & 0.6961 & 0.7860 & \textbf{0.9418} & 0.7690 & \textbf{0.8957} \\
\midrule
Real & 30 & \textbf{0.2100} & \textbf{0.7037} & \textbf{0.7971} & \textbf{0.9417} & \textbf{0.8005} & 0.8758 \\
Fake & 300 & 0.2228 & 0.6843 & 0.7797 & 0.9388 & 0.7683 & \textbf{0.8810} \\
\midrule
Real & 35 & \textbf{0.2164} & \textbf{0.6955} & \textbf{0.7889} & \textbf{0.9398} & \textbf{0.8157} & 0.8456 \\
Fake & 350 & 0.2465 & 0.6677 & 0.7543 & 0.9346 & 0.7385 & \textbf{0.8933} \\
\midrule
Real & 40 & \textbf{0.2065} & \textbf{0.7085} & \textbf{0.7974} & \textbf{0.9417} & 0.7881 & \textbf{0.8947} \\
Fake & 400 & 0.2194 & 0.6894 & 0.7816 & 0.9305 & \textbf{0.8276} & 0.8219 \\
\midrule
Real & 45 & \textbf{0.1982} & \textbf{0.7188} & \textbf{0.8062} & \textbf{0.9441} & \textbf{0.8120} & \textbf{0.8839} \\
Fake & 450 & 0.2319 & 0.6794 & 0.7697 & 0.9341 & 0.7859 & 0.8633 \\
\midrule
Real & 50 & \textbf{0.2091} & \textbf{0.7115} & \textbf{0.7948} & \textbf{0.9418} & 0.7898 & \textbf{0.8932} \\
Fake & 500 & 0.2255 & 0.6896 & 0.7756 & 0.9380 & \textbf{0.7961} & 0.8644 \\
\bottomrule
\end{tabular}
\label{tab:real_vs_fake_comparisons_with_small_datasets}
\end{table*}

==> tables/sifid.tex <==
\begin{table}[!t]
\begin{tabular}{lrll}
\begin{tabular}[c]{@{}l@{}}Target data sets\\ (1000 images)\end{tabular} & \multicolumn{1}{l}{SIFID} & Mean                           & STD             \\
Real                           & \multicolumn{1}{l}{-1.3104184E-14} & -1.3104184E-14       & N/A \\
SinGAN-Seg (No ST) - set 1     & 0.35146075                         & \multicolumn{1}{r}{} &     \\
SinGAN-Seg (No ST) - set 2     & 0.3498911                          &                      &     \\
SinGAN-Seg (No ST) - set 3                                               & 0.35274708                & \multicolumn{1}{r}{0.34974028} & 0.002492662835  \\
SinGAN-Seg (No ST) - set 4     & 0.3466186                          &                      &     \\
SinGAN-Seg (No ST) - set 5     & 0.34798387                         &                      &     \\
SinGAN-Seg (ST-1:1) - set 1    & 0.22175007                         &                      &     \\
SinGAN-Seg (ST-1:1) - set 2    & 0.2214245                          &                      &     \\
SinGAN-Seg (ST-1:1) - set 3                                              & 0.22167549                & 0.22159299                     & 0.0001405250022 \\
SinGAN-Seg (ST-1:1) - set 4    & 0.22164853                         &                      &     \\
SinGAN-Seg (ST-1:1) - set 5    & 0.22146636                         &                      &     \\
SinGAN-Seg (ST-1:1000) - set 1 & 0.22058536                         &                      &     \\
SinGAN-Seg (ST-1:1000) - set 2 & 0.22022542                         &                      &     \\
SinGAN-Seg (ST-1:1000) - set 3                                           & 0.22043976                & 0.220382674                    & 0.0001474880239 \\
SinGAN-Seg (ST-1:1000) - set 4 & 0.22041106                         &                      &     \\
SinGAN-Seg (ST-1:1000) - set 5 & 0.22025177                         &                      &    
\end{tabular}
\label{tbl:sifid}
\end{table}
